Beyond Classification: Definition and Density-based Estimation of Calibration in Object Detection

Despite their impressive predictive performance in various computer vision tasks, deep neural networks (DNNs) tend to make overly confident predictions, which hinders their widespread use in safety-critical applications. While there have been recent attempts to calibrate DNNs, most of these efforts have primarily been focused on classification tasks, thus neglecting DNN-based object detectors. Although several recent works addressed calibration for object detection and proposed differentiable penalties, none of them are consistent estimators of established concepts in calibration. In this work, we tackle the challenge of defining and estimating calibration error specifically for this task. In particular, we adapt the definition of classification calibration error to handle the nuances associated with object detection, and predictions in structured output spaces more generally. Furthermore, we propose a consistent and differentiable estimator of the detection calibration error, utilizing kernel density estimation. Our experiments demonstrate the effectiveness of our estimator against competing train-time and post-hoc calibration methods, while maintaining similar detection performance.

==> figs/laece_vs_kde_laece.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.917647058823529,0.917647058823529,0.949019607843137}
\definecolor{color1}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color2}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}
\definecolor{color3}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}

\begin{axis}[
/pgf/number format/.cd, 1000 sep={},
axis background/.style={fill=color0},
axis line style={white},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, fill=color0},
scaled x ticks = false,
scaled y ticks = false,
tick align=outside,
x grid style={white},
x tick label style={/pgf/number format/fixed},
xlabel={Number of samples},
xmajorgrids,
xmin=-395, xmax=10495,
xtick style={color=white!15!black},
xtick={-2000,0,2000,4000,6000,8000,10000,12000},
xticklabels={\ensuremath{-}2000,0,2000,4000,6000,8000,10000,12000},
y grid style={white},
y tick label style={/pgf/number format/.cd, fixed, fixed zerofill, precision=3},
ylabel={CE},
ymajorgrids,
ymin=0.0601739942499132, ymax=0.0638177025119532,
ytick style={color=white!15!black}
]
\path [draw=color1, fill=color1, opacity=0.25]
(axis cs:100,0.0636368169380921)
--(axis cs:100,0.0624101788805229)
--(axis cs:500,0.0603396173527332)
--(axis cs:1000,0.0607505048619599)
--(axis cs:3000,0.0606447669400033)
--(axis cs:5000,0.0605601758323349)
--(axis cs:8000,0.060522252216704)
--(axis cs:10000,0.0605360783296696)
--(axis cs:10000,0.0607860684734711)
--(axis cs:10000,0.0607860684734711)
--(axis cs:8000,0.0607933157237695)
--(axis cs:5000,0.0608154713548981)
--(axis cs:3000,0.0609512803422156)
--(axis cs:1000,0.0615608845842987)
--(axis cs:500,0.0615555163512139)
--(axis cs:100,0.0636368169380921)
--cycle;

\path [draw=color1, fill=color1, opacity=0.25]
(axis cs:100,0.0636520794091332)
--(axis cs:100,0.0624280148687255)
--(axis cs:500,0.0603826874230623)
--(axis cs:1000,0.0608067756894425)
--(axis cs:3000,0.0606990626127461)
--(axis cs:5000,0.0606144649434727)
--(axis cs:8000,0.0605773536124059)
--(axis cs:10000,0.0605926764507526)
--(axis cs:10000,0.0608405950169331)
--(axis cs:10000,0.0608405950169331)
--(axis cs:8000,0.0608476410052947)
--(axis cs:5000,0.0608717101167995)
--(axis cs:3000,0.061004802766349)
--(axis cs:1000,0.061612854301612)
--(axis cs:500,0.0615956461693526)
--(axis cs:100,0.0636520794091332)
--cycle;

\addplot [line width=2pt, color1]
table {%
100 0.0630234979093075
500 0.0609475668519735
1000 0.0611556947231293
3000 0.0607980236411095
5000 0.0606878235936165
8000 0.0606577839702368
10000 0.0606610734015703
};
\addlegendentry{$\laece$}
\addplot [line width=2pt, color2]
table {%
100 0.0630400471389294
500 0.0609891667962074
1000 0.0612098149955273
3000 0.0608519326895475
5000 0.0607430875301361
8000 0.0607124973088503
10000 0.0607166357338429
};
\addlegendentry{$\kde$(identity)}
\addplot [line width=2pt, color3]
table {%
100 0.0606664679944515
500 0.0606664679944515
1000 0.0606664679944515
3000 0.0606664679944515
5000 0.0606664679944515
8000 0.0606664679944515
10000 0.0606664679944515
};
\addlegendentry{Ground truth}
\end{axis}

\end{tikzpicture}

